Iterative Mode-Dropping for the Sum Capacity of MIMO-MAC with Per-Antenna Power Constraint

We propose an iterative mode-dropping algorithm that optimizes input signals to achieve the sum capacity of the MIMO-MAC with per-antenna power constraint. The algorithm successively optimizes each user's input covariance matrix by applying mode-dropping to the equivalent single-user MIMO rate maximization problem. Both analysis and simulation show fast convergence. We then use the algorithm to briefly highlight the difference in MIMO-MAC capacities under sum and per-antenna power constraints.

==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> body/Abstract.tex <==
\begin{abstract}
%=======Motivation======================

% =======General Purpose of this paper==========
%We consider the problem of maximizing the sum rate of the MIMO-MAC with per-antenna power constraint. 
% =======How to solve this problem ======
%An efficient algorithm is proposed to compute optimal input covariance matrices and sum capacity.
We propose an iterative mode-dropping algorithm that optimizes input signals to achieve the sum capacity of the MIMO-MAC with per-antenna power constraint.
% =======Numerical issue==============
%The numerical algorithm is similar iterative water-filling for MIMO MAC with sum power constraint and iteratively maximizing the sum-rate objective by successively solving single-user MIMO optimization problem with per-antenna power constraint.
%In a way similar to iterative water-filling under sum power constraint, 
%It successively optimizes one of these matrices by
%applying mode-dropping to the equivalent single-user MIMO rate maximization problems.
%The algorithm converges to the sum capacity fast and precisely.
The algorithm successively optimizes each user's input covariance matrix by applying mode-dropping to the equivalent single-user MIMO rate maximization problem.
Both analysis and simulation show fast convergence. We then use the algorithm to briefly highlight the difference in MIMO-MAC capacities under sum and per-antenna power constraints.
%is based on the single-user MIMO rate optimization with per-antenna power constraint and 
%% =======Results: This turn out to be good==================
%The algorithm converges to the sum capacity fast and precisely.
%We also compare the capacity of MIMO-MAC under per-antenna power constraint with that under sum power constraint.
%and shows that with equal constraint per antenna, sum capacity can be close to the capacity with sum power constraint.
\end{abstract}
%tractable, controllable, and conceptual clear, 
\begin{IEEEkeywords}
Multiple-access channels (MAC), Multiuser MIMO, per-antenna power, sum capacity
\end{IEEEkeywords}

%========================= Old Abstract =======================%
%Important theoretical considerations: computation complexity, least square error, Gibbs effects, adaptivity and integral approximations and physical insights.
%
%Things done:
%\begin{enumerate}
%\item Formulate optimization algorithms
%\begin{itemize}
%\item
%Solution discussion with Normal Equation
%\item
%Algorithm formulation for minimal filter order 
%\begin{itemize}\item 
%Approximate the integration\item 
%Derive the algorithms by exploring the Toeplitz and symmetry characteristics of the matrix 
%\end{itemize}
%\end{itemize}
%\item SVD for analysis of the solution
%\begin{itemize}\item 
%SVD decomposition\item 
%DPSWF and DPSS related derivations (partly)
%\end{itemize}
%\item Derivation of error from rectangular window and IFFT
%\end{enumerate}
%Things to do:
%\begin{enumerate}
%\item Discuss the filter order based on DPSWF and DPSS
%\begin{itemize}
%\item
%Derive the required filter order approximately
%\item
%Formulate the optimization of step size with overall computational complexity
%\end{itemize}
%\item Derivation of error from two Turkey windowing method
%\item Numerical Analysis
%\end{enumerate}


%
%\item  Windowing FIR Filter Design
%\begin{itemize}
%\item 
%Investigate the effects of windowing on the integral approximation
%\item 
%Formulate the error function with approximation 
%\item
%Get an analytical expression for optimal window parameter
%\end{itemize}
%\item 
%Comparison of different algorithms: complexity and accuracy 
%\item
%Extension to variable step size case
%\begin{itemize}\item
%Validate the relationship between FIR coefficients of different step size \item
%Joint optimization of filter design error and step-size induced error
%\end{itemize}
%\item
%Extension to other frequency dependent effects, eg. PMD
%\begin{itemize}\item
%Drive the approximation of several PMD matrix multiplication \item
%Design PMD-dispersion joint FIR coefficients extraction
%\end{itemize}
%\item
%Apply the algorithms to split-step simulation of fiber or backpropagation


==> body/Conclusion.tex <==
\section{Conclusion}
\label{sec:C}
In this letter,
we have proposed an iterative mode-dropping algorithm to 
compute the sum capacity of the MIMO-MAC with per-antenna power constraint.
It successively optimizes
each user's transmit covariance matrix until convergence. %while keeping the other matrices invariant,
Similar to iterative waterfilling, iterative mode-dropping is fully distributive and has fast convergence.
The algorithm is attractive for its simplicity, low complexity and practicality when compared to general  convex programing methods. 
%in our simulations, the sum rate after the first iteration is in proximity to the sum capacity  and the gap falls below $0.1$ 

Simulations results illustrate
the difference in the sum capacity of MIMO-MAC
under per-antenna or sum power constraints.
Both of them are significantly higher than the sum rate under independent spatial multiplexing in which the input signals are non-optimized.
%The degree of freedom is limited by $\min(m, nK)$
%and increasing $n$ ($m$) when $m<nK$ ($m>nK$) can obtain a better diversity gain.
This gain in sum capacity, however, saturates with the number of users as the multiple access interference increases even under per-antenna power constraint. 
Increasing the number of antennas can increase the sum capacity as well as the capacity gain by having better degree of freedom gain, diversity gain or array gain.


%
%In this letter,
%we proposed the iterative mode-dropping algorithm to compute the sum capacity of MIMO-MAC with per-antenna power constraint.
%The rate maximization problem was solved in an iterative manner, 
%by optimizing one of the transmit covariance matrix while keeping the other matrices invariant,
%based on the single-user mode-dropping algorithm.
%We proved its convergence and showed the fast speed of convergence.

%We found that the capacity region of MIMO-MAC under per-antenna power constraint and is compared to the case of sum power constraint. The capacity region of the former is inside and can be very close to that of the latter.










==> body/ConvergenceAnalysis.tex <==
%\section{Iterative Algorithms and Convergence Analysis}
%\label{sec:IACA}
%\subsection{Iterative Mode-Dropping Algorithm}
%
%\subsection{Convergence Analysis}
%
%\subsection{Connections with Iterative Water-Filling}








==> body/Intro.tex <==
\section{Introduction}
\label{sec:intro}
%\IEEEPARstart{M}
%IMO channels have been widely investigated in the past decades as they provides enormous information rates in wireless networks.
\IEEEPARstart{U}{}nder sum power constraint, the capacity of MIMO channels has already been well-established.
With channel state information (CSI) available at both the transmitter and the receiver, the single-user capacity is achieved by diagonalizing the channel matrix then water-filling the total power across the spatial subchannels \cite{telatar1999capacity}. % eigenmodes.
Based on this single-user water-filling algorithm, the sum capacity of the MIMO multiple access channel (MIMO-MAC) can be efficiently computed in an iterative manner, by optimizing the transmit covariance matrix of each user successively while treating the signals from all other users as noise\cite{yu2004iterative}.
%Single-user water-filling can be generalized to iterative water-filling which efficiently finds the optimal signaling and computes the sum capacity of MIMO-MAC \cite{yu2004iterative}.\

Sum power constraint is, however, less practical than per-antenna constraint because the power amplifier at each antenna has 
its own output dynamic range \cite{yu2007transmitter}.
%However, the sum power constraint is less practical than per-antenna constraint.
%Because each antenna has its own amplifier and its power is limited individually by the output dynamic range of the amplifier, power sharing among different antennas is difficult\cite{yu2007transmitter}.
The capacity under this per-antenna power constraint has been investigated for different channel models.
For single-user MISO channels, the capacity can be expressed in closed form and is achieved by a single-mode beamformer,
with its phase matched to that of the channel vector and its amplitude determined by the power constraint \cite{vu2011miso}.
%whose phase is matched to that of the channel vector and amplitude is determined by individual power constraint \cite{vu2011miso}.
%For single-user MIMO channels, 
%the capacity is computed by solving  the KKT optimal conditions
%based on an adaptive \emph{mode-dropping} algorithm \cite{vu2011capacity}.
For single-user MIMO channels, the capacity optimization problem can be formulated in 
the framework of semidefinite programming and a simple adaptive \emph{mode-dropping} algorithm computes the capacity by solving the Karush-Kuhn-Tucker (KKT) conditions efficiently
% and also provides some physical insights 
\cite{vu2011capacity}.
For the MIMO-MAC, although the sum-rate maximization problem is convex
and hence readily solvable using %general methodologies such as 
interior-point methods, 
the computational complexity could be impractically high when the system has a large number of users or antennas. 

In this regard, we propose a more efficient algorithm called \emph{iterative mode-dropping} to find the optimal transmit covariance matrices
that achieve the sum capacity of the MIMO-MAC with per-antenna power constraint.
In a way similar to the iterative water-filling algorithm \cite{yu2004iterative}, 
iterative mode-dropping optimizes the transmit covariance matrices successively.
In each step, 
it optimizes the covariance matrix of one user based on the mode-dropping algorithm for single-user MIMO channels,
while holding those of the other users constant.
The algorithm converges surely to the sum capacity and simulation results show fast convergence, typically 
within $10^{-6}$ bps/Hz of the sum capacity
after $10$ iterations (i.e., each user has updated its covariance matrix $10$ times).  
We also use the algorithm to compare the sum capacity under different power constraints and study the effects on capacity of SNR, the number of users and the number of antennas.

%The rest of the paper is organized as follows. In Section II, we present the channel model and review the capacity under sum power constraint. The single-user mode-dropping is introduced and the extension to MIMO-MAC is shown in Section III The numerical validation and analysis are given in Section IV, followed by the conclusion remarks in Section V. 

The following notation is used: an italic letter, boldface lowercase or boldface uppercase letter represents a scalar, column vector or matrix, respectively. $(\cdot)^T$ or $(\cdot)^{\dagger}$ denotes transpose or conjugate transpose of a matrix. 
Tr$(\cdot)$ is the trace and $\det(\cdot)$ is the determinant of a matrix. 
The operator $\succcurlyeq$ and $\preccurlyeq$ represent positive semidefinite ordering of Hermitian matrices.
diag$\{\cdot\}$ or diag$(\cdot)$ forms a diagonal matrix with given entries or from the diagonal entries of the given matrix, respectively. $\mathbf I$ is an identity matrix of appropriate dimension.








==> body/NumericalAnalysis.tex <==
\section{Numerical Examples}
\label{sec:NR}

In this section, we numerically investigate the convergence behavior of iterative mode-dropping and quantify the difference between the MIMO-MAC capacities under the per-antenna and the sum power constraints. 
Throughout this section, we assume that the wireless channels undergo independent Rayleigh fading,
that is,
the entries of the channel matrices are i.i.d. % independent and identically distributed as 
circularly symmetric complex Gaussian variables with zero mean and unit variance. 
The ergodic capacity is computed by averaging over $2000$ channel realizations.

\begin{figure}[!t]
\centering
\includegraphics[width=0.5\textwidth]{Fig1}
\caption{Convergence examples of the sum rate under per-antenna power constraint (iterative mode-dropping) and sum power constraint (iterative water-filling).}
\label{convergence}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=0.5\textwidth]{Fig2}
\caption{The expected number of single-user mode-dropping iterations required to reach within $10^{-6}$ bps/Hz of sum capacity, together with the standard deviation.}
\label{complexity}
\end{figure}


In Figure~\ref{convergence}, 
we compare convergence behaviors of iterative mode-dropping and iterative water-filling.
Consider a system of $K=15$ users with two different antenna settings: $n=4,m=4$ and $n=8,m=4$. 
For each user, the per-antenna power constraint is set to $0.5$ for $n=4$ and $0.25$ for $n=8$ and the sum power constraint is set to $2$. 
Figure~\ref{convergence} shows the ergodic sum rate versus the number of iterations 
for both power constraints.
After the first iteration, the sum rates are already very close to the sum capacity, and
after the second iteration, the gap to optimality is lower than $10^{-1}$ for both constraints. 
The same convergence behavior can be observed for all simulations that we ran.
In addition, the higher capacity achieved with more transmit antennas is attributed to the diversity gain and array gain. 
In Figure~\ref{complexity}, the expected number of single-user mode-dropping iterations required to reach within $10^{-6}$ bps/Hz of the sum capacity versus the number of users is shown together with the corresponding standard deviation.
Here we let $n = m = 4$, the per-antenna constraint be $0.5$, and use
$500$ random channel realizations to generate these statistics.
This result verifies Remark 3 that the total complexity grows linearly with the number of users $K$.
%We note that the speed of convergence may vary for different channel realizations.

\begin{figure}[!t]
\centering
\includegraphics[width=0.5\textwidth]{Fig3}
\caption{Sum capacities and bounds on the capacity region of the two-user MIMO-MAC under per-antenna or sum power constraint.}
\label{twouser}
\end{figure}

Figure~\ref{twouser} presents the capacity region of a two-user MIMO-MAC for the two different power constraints.
The numbers of antennas are $n=m=4$, 
the sum power constraint is $2$ per user and 
the per-antenna constraint is $0.5$.
The first iteration of all the transmit covariance matrices
leads to $\{\mathbf Q_{1}^{\mathrm{A}},
\mathbf Q_{2}^{\mathrm{A}} \}$ that can achieve the point A if $\mathbf Q_{2}$ is updated before $\mathbf Q_{1}$,
and $\{\mathbf Q_{1}^{\mathrm{B}},
\mathbf Q_{2}^{\mathrm{B}} \}$ that can achieve the point B vice versa.
Iterative mode-dropping converges to both point C and point D,  which give the sum capacity line CD.
The inner-bound curve AC 
corresponds to rate region achieved
by the convex hull 
 $\{ \mu \mathbf Q_{1}^{\mathrm{A}} + (1-\mu) \mathbf Q_{1}^{\mathrm{C}},
 \mu \mathbf Q_{2}^{\mathrm{A}} + (1-\mu) \mathbf Q_{2}^{\mathrm{C}} \}$ with $0 \leq \mu \leq 1$,
similar for the curve BD.
The piecewise outer bound comprises of 
three line segments that are defined by
the single-user capacities and the sum capacity.
%The capacity region must lie below the line passing through C and D.
%As expected, the capacity region with per-antenna power is inside that with sum power. 
The proposed algorithm converges precisely to the sum capacity with per-antenna constraint and can provide computationally simple inner and outer bounds to the capacity regions.
In addition, 
this figure illustrates the difference between the capacity regions under the two power constraints.


%However, the outer bound of per-antenna power case can be very close to the inner bound of sum power constraint
% at the conner points.

Figure~\ref{capacitygap} compares the sum capacities under the following scenarios:
1) sum power constraint;
2) per-antenna constraint with equal power across antennas;
3) per-antenna constraint with unequal power, in which the power of the $k$th antenna is proportional to $k$;
4) spatial multiplexing with equal substreams, that is, the transmit covariance matrices $\mathbf Q_i$'s are proportional to $\mathbf I$; and 5) spatial multiplexing with unequal substreams, in which $\mathbf Q_i$'s are diagonal, with the $k$th diagonal entry proportional to $k$.
%The SNR is defined as the ratio of the per-user signal power and the per-antenna noise power.
We also plot the capacity gaps between the sum power and the per-antenna power constraints (equal or unequal),
and between the per-antenna constraints (equal or unequal) and the corresponding independent spatial multiplexing.
The parameters are chosen as $K=4$, $m=4$, and $n=4,8$.

\begin{figure}[!t]
\centering
\includegraphics[width=0.5\textwidth]{Fig4}
\caption{Comparison of the ergodic sum capacity versus per-user SNR for different scenarios.
%with sum power constraint, with per-antenna power constraint (equal or unequal power distribution), and spatial multiplexing (independent substreams). 
The insetted figures show the capacity gaps between the per-antenna constraint and independent spatial multiplexing (left), and between the sum power and per-antenna power constraints (right).
Parameters: $K=4, m=4$ and $n=4, 8$.}
\label{capacitygap}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=0.5\textwidth]{Fig5}
\caption{Ergodic sum capacity versus the number of users under sum power constraint, per-antenna power constraint and independent spatial multiplexing. For the per-antenna power constraint, the sum rate after the first iteration is also included. The insetted figures show the capacity gaps between the sum power and per-antenna constraints (left), and 
between the per-antenna constraint and independent spatial multiplexing (right).}
\label{vsUsers}
\end{figure}

The following observations can be made:
First, as expected, the decreasing order of capacity is under sum power, per-antenna (equal power), per-antenna (unequal power),
independent spatial multiplexing (equal power) and independent spatial multiplexing (unequal power).
Our simulations provide a quantitative example of the difference between MIMO-MAC capacities under per-antenna constraint or sum power constraint,
and show that both are significantly higher than the sum rate under independent spatial multiplexing in which $\mathbf Q_i $'s are not at all optimized.
%The first three outperform the last two by a wide margin.
Second, as the number of transmit antennas $n$ increases,
the increase in sum capacity under any of the first three power constraints is significantly more than
that under independent spatial multiplexing.
Additional transmit antennas provide a better diversity gain,
and iterative waterfilling and iterative mode-dropping both 
attempt to minimize the effects of multiple access interference,
whereas independent spatial multiplexing does not.
Hence the capacity gap (compared to independent spatial multiplexing) increases with the number of transmit antennas. 


Last, as illustrated in Figure~\ref{vsUsers}, the sum capacity under sum power constraint, per-antenna power constraint and independent spatial multiplexing increases with the number of users $K$.
The capacity gaps also increase with $K$ and the number of antennas.
As $K$ increases, however,  the capacity gaps become saturated
because the system is more interference-limited.
As the number of antennas increases 
(from $n=m=2$ to $n=m=8$) the capacity increases due to the degree of freedom gain.
Furthermore, after just one iteration, the sum rate obtained by iterative-mode dropping is already in good proximity with the true capacity.





==> body/Problemformulate.tex <==
\section{System Model and Known Capacity}
\label{sec:SM}
\subsection{MIMO-MAC model and per-antenna power constraint}
A $K$-user Gaussian MIMO-MAC with $n$ antennas at each transmitter and $m$ antennas at the receiver can be modeled as
\begin{IEEEeqnarray}{rCl}
\label{systemmodel} 
\mathbf{y}=\sum_{i=1}^{K}\mathbf{H}_{i}\mathbf{x}_{i}+\mathbf{z} \; ,
\end{IEEEeqnarray}
where vector $\mathbf{x}_{i}\in \mathbb{C}^{n\times1}$ is the transmitted signal of the $i$th user, vector $\mathbf{y}\in \mathbb{C}^{m\times1}$ is the received signal, $\mathbf{H}_{i}\in \mathbb{C}^{m\times n}$ is the channel matrix from the $i$th user to the receiver, and vector $\mathbf{z}\sim \mathcal{CN} (\mathbf 0,\mathbf{I})$ is the additive circularly symmetric complex Gaussian noise at the receiver\footnote{Without loss of generality, we assume that this noise vector is spatially white and has been normalized.}.
%Here we consider zero-mean Gaussian input singles. 
We assume that the channel matrices are full-rank and perfect CSI is available at all transmitters and the receiver.

In this model, we consider a per-antenna power constraint in which each transmit antenna has its own power budget and the antennas of the same user can cooperate in terms of signaling. 
Considering zero-mean input signals, 
 $\mathbf{Q}_{i}=E[\mathbf{x}_i\mathbf{x}_i^{\dagger}]$ is the transmit covariance matrix of the $i$th user. Hence, the set of covariance matrices $\{\mathbf{Q}_i\}$ satisfies 
\begin{IEEEeqnarray}{rCl}
\label{perantennapower} 
\text{diag}(\mathbf{Q}_i) \preccurlyeq \mathbf{P}_i, \quad \forall i=1,\cdots,K\; ,
\end{IEEEeqnarray}
where $\mathbf{P}_i=\text{diag}\{P_{i1}, P_{i2},\cdots,P_{in}\}$ and $P_{ij}$ is the power constraint for the $j$th antenna of the $i$th user.

\subsection{Review of the capacity with sum power constraint}
%The sum capacity of MIMO-MAC is well-studied under sum power constraint. 
%Here, we consider a more practical model of per-antenna power constraint.
%For comparison, the sum power constraint is included and elaborated below along with the review of 
%the capacity results.
For comparison, the sum power constraint and the corresponding MIMO-MAC capacity are summarized here.
In this scenario, the $i$th user has the total transmit power across all its antennas constrained by $P_i$, that is,
\begin{IEEEeqnarray}{rCl}
\label{sumpowerconstraint} 
\text{tr}(\mathbf{Q}_i)\leq P_i, \quad i=1,\cdots,K\; .
\end{IEEEeqnarray}
To achieve sum capacity, the users choose their positive semidefinite transmit covariance matrices, $\{ \mathbf Q_i \}$,
to maximize the sum rate of the MIMO-MAC subject to the above power constraints.

This problem can be solved efficiently by iterative water-filling\cite{yu2004iterative}.
%In this scenario, the total power of the $i$th user across all its antennas has a ceiling of $P_i$, that is,
%\begin{IEEEeqnarray}{rCl}
%\label{sumpowerconstraint} 
%\text{tr}(\mathbf{Q}_i)\leq P_i, \quad i=1,\cdots,K\; .
%\end{IEEEeqnarray}
%The users can choose their positive semidefinite transmit covariance matrices, $\{ \mathbf Q_i \}$,
%to maximize the sum rate of the MIMO-MAC subject to the above power constraints.
The underlying principle is to successively update each one of the $K$ covariance matrices, say $\mathbf Q_k$, by keeping all other $K-1$ matrices at the other users unchanged. 
In each step, the subproblem is equivalent to a single-user rate maximization problem
by treating other users' signals as noise,
for which water-filling is readily applicable.
This algorithm converges surely to the sum capacity and the rate of convergence is fast.
%More specifically, after just one iteration for $\{ \mathbf Q_i \}$, the rate per user per output dimension is at most $1/2$ nats away from the sum capacity. 
%The simplicity and its convergence property enables a real time implementation.

%
%, the sum power constraint is included and elaborated below along with the review of known capacity results.
%Under sum power constraint, the total power of $i$th user across $n$ antennas is $P_i$. As all the antennas at each transmitter can cooperate, each user can choose its signal beam-forming vector subject to the constraint on the input covariance matrix, as follows
%\begin{IEEEeqnarray}{rCl}
%\label{sumpowerconstraint} 
%\text{tr}(\mathbf{Q}_i)\leq P_i, \quad i=1,\cdots,K\; .
%\end{IEEEeqnarray}
%%Therefore, the sum rate optimization problem of MIMO MAC is formulated as
%%\begin{IEEEeqnarray}{rCl}
%%\label{sumpowerMAC} 
%%\max \quad&&\log \det (\mathbf{I}_m+\sum_{i=1}^{K}\mathbf{H}_{i}\mathbf{Q}_{i}\mathbf{H}_{i}^{\dagger}) \nonumber \\
%%\text{s.t.} \quad&&\text{tr}(\mathbf{Q}_i)\leq P_i, \quad i=1,\cdots,K\nonumber \\
%%&&\mathbf{Q}_i \succcurlyeq 0,\quad \quad \quad i=1,\cdots,K \;, 
%%\end{IEEEeqnarray}
%%where $\mathbf{Q}_i$ is Hermitian. 
%
%%Notice that the problem is convex and the constraints for different users are separable, the global optimum can be found by iteratively optimize the objective function with respect to one variable while keeping all other variables as constant. The iteration repeats until the sum rate converges to the optimal value. 
%The efficient solution to this problem is iterative water-filling\cite{yu2004iterative}.
%In each iteration, each of the $K$ covariance matrix is updated successively by holding the covariance matrix of other $K-1$ users invariant. As in each step the procedure of $k$th covariance update can be valued as a single-user rate optimization problem and single-user optimization problem can be obtained in closed-form using water-filling, the algorithm is simple in calculation. The convergence is very fast. More specifically, after just one iteration, the capacity loss per user per output dimension is at most $1/2$ nats from the sum capacity. The simplicity and its convergence property enables a real time implementation.







==> body/SumRate.tex <==
\section{Sum Rate Maximization with Per-Antenna Power Constraint}
\label{sec:SRM}

%
%
%\begin{algorithm}
%Initialize $\mathbf{D}_1^{0}\succ \mathbf 0$, $\mathbf{P}_1\succ \mathbf 0$, $\epsilon>0$, iteration count $i=0$, and terminating variable $\Delta=1+\epsilon$.  \\
%$\mathbf{if}$ $n\leq m$, $\mathbf{then}$\\
%\quad  $\mathbf{repeat}$\\
%\quad \qquad $-\mathbf{S}_n^{i}=\text{non-positive eigenmodes of } \mathbf{K}(\mathbf{D}_1^{i})^{-1}\mathbf{K}^{\dagger}-\mathbf{I}_n$ \\
%\quad \qquad $\mathbf{Z}^{i}=\mathbf{K}^{-1}\mathbf{S}_n^{i}(\mathbf{K}^{-1})^{\dagger}\n $\\
%\quad \qquad $\mathbf{Q}_{1}^{i}=(\mathbf{D}_1^{i})^{-1}-\mathbf{K}^{-1}(\mathbf{K}^{-1})^{\dagger}+\mathbf{Z}^{i}$ \\
%\quad \qquad $\mathbf{D}_{1}^{i+1}=\mathbf{D}_1^{i}+\mathbf{P}_{1}-\text{diag} (\mathbf{Q}_1^{i})$\\
%\quad \qquad $\Delta = |\text{tr}[\mathbf{D}_1^{i}(\mathbf{Q}_{1}^{i}-\mathbf{P}_{1})]|$\\
%\quad \qquad $i=i+1$ \\
%\quad $\mathbf{until}$\text{ }the $\Delta \leq \epsilon$.\\
%$\mathbf{else}$\\
%\quad $\mathbf{repeat}$\\
%\quad \qquad $-\mathbf{S}_m^{i}=\text{non-positive eigenmodes of } \mathbf{H}_{1}(\mathbf{D}_1^{i})^{-1}\mathbf{H}_{1}^{\dagger}-\mathbf{I}_m$\\
%\quad \qquad $\mathbf{Z}^{i}=\mathbf{H}^{-1}\mathbf{S}_m^{i}(\mathbf{H}^{-1})^{\dagger}$ \\
%\quad \qquad $\mathbf{X}^{i}=\mathbf{V}_2\mathbf{A}^{i}\mathbf{V}_2^{\dagger}+\mathbf{V}_1\mathbf{B}^{i}\mathbf{V}_2^{\dagger}+\mathbf{V}_2\mathbf{B}^{i}\mathbf{V}_1^{\dagger}$ \\
%\quad \qquad $\mathbf{Q}_{1}^{i}=(\mathbf{D}_1^{i})^{-1}-\mathbf{H}^{-1}(\mathbf{H}^{-1})^{\dagger}+\mathbf{Z}^{i}-\mathbf{X}^{i}$ \\
%\quad \qquad $\mathbf{D}_{1}^{i+1}=\mathbf{D}_1^{i}+\mathbf{P}_{1}-\text{diag} (\mathbf{Q}_1^{i})$\\
%\quad \qquad $\Delta = |\text{tr}[\mathbf{D}_1^{i}(\mathbf{Q}_{1}^{i}-\mathbf{P}_{1})]|$\\
%\quad \qquad $i=i+1$ \\
%\quad $\mathbf{until}$\text{ }the $\Delta\leq \epsilon$.
%\caption{Single-user mode-dropping  for solving
%$\mathbf{Q}_1^{\ast} = 
%\underset{{\text{diag}(\mathbf{Q})\preccurlyeq \mathbf{P}_1, \mathbf{Q} \succcurlyeq \mathbf 0}}{\arg \max}
% \log \det (\mathbf{\hat{H}}_{1}\mathbf{Q}\mathbf{\hat{H}}_{1}^{\dagger}+\mathbf{I}_m)
%$}
%\end{algorithm}



The sum-rate maximization problem for MIMO-MAC with per-antenna power constraint can be formulated as a convex optimization problem of $\{\mathbf{Q}_i\}$:
\begin{IEEEeqnarray}{rCl}
\label{perantennapowerMAC} 
\max_{\{\mathbf{Q}_i\}} \quad&&\log \det \Big(\mathbf{I}_m+\sum_{i=1}^{K}\mathbf{H}_{i}\mathbf{Q}_{i}\mathbf{H}_{i}^{\dagger}\Big)  \\
\text{s.t.} \quad&&\text{diag}(\mathbf{Q}_i) \preccurlyeq \mathbf{P}_i, \quad i=1,\cdots,K\nonumber \\
&&\mathbf{Q}_i \succcurlyeq \mathbf 0,\quad \quad \quad\quad i=1,\cdots,K \nonumber \;.
\end{IEEEeqnarray}
%The sum capacity with sum power constraint is no less than that with per-antenna power constraint because the feasible region of the former optimization problem includes that of the latter as a subset.
The sum capacity with per-antenna power constraint is usually less than that with sum power since the feasible region of the former optimization problem is included in the latter as a subset.
%%where $\{\mathbf{Q}_i\}$ is the set of input covariance matrices of $K$ users we want to optimize to find the sum capacity. 
%The optimal $\{\mathbf{Q}_i\}$ always satisfy the equality, $\text{diag}(\mathbf{Q}_i) = \mathbf{P}_i$; otherwise, we can always increase the power of antennas and thus obtain a higher sum rate. 
%This problem is convex in $\{\mathbf{Q}_i\}$ and thus can be solved using general methodologies such as interior-point methods. %However, the efficient way for computing capacity is still missing.
Unfortunately, no closed-form solution has been found for this problem. Inspired by iterative water-filling, we propose an iterative mode-dropping algorithm to solve this problem efficiently.  
Before presenting this algorithm,  it is necessary to briefly review mode-dropping for single-user MIMO channels as in \cite{vu2011capacity}.


\subsection{Single-user mode-dropping}
%For single-user MIMO channel with per-antenna power constraint, the capacity optimization problem can be posed as follows,
%\begin{IEEEeqnarray}{rCl}
%\label{singleusermodedropping} 
%\max_{\mathbf{Q}} \quad&&\log \det (\mathbf{I}_m+\mathbf{H}\mathbf{Q}\mathbf{H}^{\dagger}) \nonumber \\
%\text{s.t.} \quad&&\text{diag}(\mathbf{Q}) \preccurlyeq \mathbf{P}\nonumber \\
%&&\mathbf{Q} \succcurlyeq 0 \;,
%\end{IEEEeqnarray}
%where $\mathbf{P}=\text{diag}\{P_{1}, P_{2},\cdots,P_{n}\}$ and $P_{i}$ is the power constraint for the $i$th antenna.
%The capacity optimization problem for single-user MIMO channel with per-antenna power constraint is  given by setting $K=1$ in (\ref{perantennapowerMAC}). 
The problem in (\ref{perantennapowerMAC}) reduces to the scenario of single-user MIMO channels when $K=1$.
%Because Slater's condition is satisfied, the Karush-Kuhn-Tucker (KKT) condition is sufficient and necessary for optimality. 
%The Lagrangian of the problem in (\ref{singleusermodedropping}) is 
%\begin{IEEEeqnarray}{rCl}
%\label{singleLagrangian} 
%\mathcal{L}(Q,D,M)=\log \det(&&\mathbf{I}_m+\mathbf{H}\mathbf{Q}\mathbf{H}^{\dagger}) \nonumber \\
%&& - \text{tr}[\mathbf{(D(Q-P)}]+\text{tr}(\mathbf{MQ})\;,
%\end{IEEEeqnarray}
The KKT conditions are necessary and sufficient for optimality because Slater's condition is satisfied, and the objective function and inequality constraints are continuously differentiable and concave functions of $\{\mathbf{Q}_i\}$. 
%Therefore, the optimal point can be found by solving the KKT conditions.
Based on the KKT conditions,  a set of single-user optimality conditions can be stated as follows.
%\begin{IEEEeqnarray}{rCl}
%\label{singleKKT} 
%\label{singleKKT1}
%\mathbf{H}^{\dagger}(\mathbf{I}_m+\mathbf{H}\mathbf{Q}\mathbf{H}^{\dagger})^{-1}\mathbf{H}&=&\mathbf{D}-\mathbf{M} \\
%\label{singleKKT2}
%\mathbf{MQ}&=&\mathbf{0} \nonumber \\
%\label{singleKKT3} 
%\text{diag}(\mathbf{Q})&=&\mathbf{P}\nonumber \\
%\label{singleKKT4}
%\mathbf{M}, \mathbf{Q} &\succcurlyeq& 0\nonumber \\
%\text{diagonal } \mathbf{D}&\succ& 0\nonumber \;,
%\end{IEEEeqnarray}
%where $\mathbf{D}$ is dual variable associated with per-antenna power constraint and positive semidefinite squared matrix $\mathbf{M}$ is the dual variable associated with positive semidefinite constraint. At optimal point, the third equality in (\ref{singleKKT1}) alway holds, otherwise we can increase the power of antennas to obtain a higher rate.
%Accordingly,  $\mathbf{D}$ is strictly positive 
%It also noticed that replacing $\mathbf{I}_m$ with any matrix that is not the function of $\mathbf{Q}$ in the objective function only changes identity matrix in (\ref{singleKKT1}) to the corresponding matrix.
\begin{IEEEeqnarray}{rCl}
\label{singleKKT} 
\label{singleKKT1}
\mathbf{H}_1^{\dagger}(\mathbf{I}_m+\mathbf{H}_1\mathbf{Q}_{1}^{\ast}\mathbf{H}_1^{\dagger})^{-1}\mathbf{H}_1&=&\mathbf{D}_{1}-\mathbf{M}_{1} \\
\label{singleKKT2}
\mathbf{M}_{1}\mathbf{Q}_{1}^{\ast}&=&\mathbf{0} \nonumber \\
\label{singleKKT3} 
\text{diag}(\mathbf{Q}_{1}^{\ast})&=&\mathbf{P}_{1}\nonumber \\
\label{singleKKT4}
\mathbf{M}_{1}, \mathbf{Q}_{1}^{\ast} &\succcurlyeq& \mathbf 0\nonumber \\
\text{diagonal } \mathbf{D}_{1}&\succ& \mathbf 0\nonumber \;,
\end{IEEEeqnarray}
where positive-definite diagonal matrix $\mathbf{D}_{1}\in \mathbb{C}^{n\times n}$ is the dual variable associated with the per-antenna power constraint and Hermitian positive semidefinite matrix $\mathbf{M}_{1}\in \mathbb{C}^{n\times n}$ is the dual variable associated with the positive semidefinite constraint. 
The covariance matrix $\mathbf{Q}_{1}^{\ast}$ satisfying the optimality conditions in (\ref{singleKKT1}) is the optimal solution that achieves the single-user MIMO capacity.
%At optimal point, the third equality in (\ref{singleKKT1}) alway holds, otherwise we can increase the power of antennas to obtain a higher rate.
%Accordingly,  $\mathbf{D}$ is strictly positive 

%Based on the above optimal conditions, the dual variable $\mathbf{M}$ can be eliminated and the covariance matrix can be written in closed-forms as a function of dual variable $\mathbf{D}$. Combined with the third the condition above, the optimal covariance matrix can be found by the adaptive algorithm, \emph{mode-dropping}, which converges to the optimal point.

The most important and challenging step of mode-dropping is 
to express $\mathbf{Q}_{1}^{\ast}$ as a function of $\mathbf{D}_{1}$
by eliminating $\mathbf{M}_{1}$ in the optimality conditions.
%Using this technique, the algorithm finds the optimal solution in an iterative procedure,
%namely, 
%to compute $\mathbf{Q}_{1}^{\ast}$ from $\mathbf{D}_{1}$,
 %update $\mathbf{D}_{1}$ based on the new $\mathbf{Q}_{1}^{\ast}$ and repeat
%until the duality gap converges to zero.
In \cite{vu2011capacity}, closed-form solution for $\mathbf{Q}_{1}^{\ast}$ in terms of $\mathbf{D}_{1}$ is established for all channel sizes. Using this solution, the remaining step is to find the optimal dual variable $\mathbf{D}_{1}$ such that the established solution satisfies the power constraint. To arrive at this optimal value, an iterative algorithm is proposed to update $\mathbf{D}_{1}$ at each step until the duality gap converges to within a specified tolerance. 
Due to space limitation,
we summarize the main steps of this algorithm as follows:
\begin{enumerate}
\item \emph{Compute $\mathbf{Q}_{1}^{\ast}$ from $\mathbf{D}_{1}$:}
Let the singular value decomposition (SVD) of the channel matrix be $\mathbf{H}_1=\mathbf{U}_{\mathbf{H}}\mathbf{\Sigma}_\mathbf{H}\mathbf{V}_\mathbf{H}^{\dagger}$. 
If $m \geq n$, let $\mathbf{\Sigma}_\mathbf{H} = [\mathbf{\Sigma}_n, \mathbf {0}_{n,m-n}]^T$ and form
\begin{itemize}
\item $\mathbf{K}=\mathbf{V}_\mathbf{H} {\mathbf{\Sigma}}_n \mathbf{V}_\mathbf{H}^{\dagger}$,
$\mathbf{K}^{-1}=\mathbf{V}_\mathbf{H} {\mathbf{\Sigma}}_n^{-1} \mathbf{V}_\mathbf{H}^{\dagger}$.
%\item   Let $\mathbf{K}\mathbf{D}_1^{-1}\mathbf{K}^{\dagger}-\mathbf{I}_n =
%\mathbf V_{\mathbf K} \mathbf{\Sigma}_{\mathbf K} \mathbf V_{\mathbf K}^{\dagger}$ be the
%eigenvalue decomposition (EVD).
%Define $(-\mathbf{S}_n)$ as the non-positive eigenmodes, that is, $\mathbf V_{\mathbf K} \min(\mathbf{\Sigma}_{\mathbf K}, \mathbf 0)\mathbf V_{\mathbf K}^{\dagger}$, where $\min()$ is an entry-wise function.
%Herein, the positive modes are \emph{dropped}.
\item $\mathbf{F}_{n}=\mathbf{K}\mathbf{D}_{1}^{-1}\mathbf{K}^{\dagger}$.
\item $-\mathbf{S}_{n}=$ non-positive eigenmodes of $(\mathbf{F}_{n}-\mathbf{I}_{n})$, here the modes contained in $\mathbf{S}_n$ are dropped.
\item $\mathbf{Z}=\mathbf{K}^{-1}\mathbf{S}_n(\mathbf{K}^{-1})^{\dagger}$.
\item $\mathbf{Q}_{1}^{\ast}=\mathbf{D}_1^{-1}-\mathbf{K}^{-1}(\mathbf{K}^{-1})^{\dagger}+\mathbf{Z}$.
\end{itemize}
If $m < n$, let  $\mathbf{\Sigma}_\mathbf{H} = [\mathbf{\Sigma}_m, \mathbf{0}_{m,n-m}]$
and $\mathbf{V}_1$ be the first $m$ columns of $\mathbf{V}_\mathbf{H}$ (i.e., write $\mathbf{V}_\mathbf{H}=[\mathbf{V}_1 \;\; \mathbf{V}_2]$). 
\begin{itemize}
\item Define the pseudo inverse of $\mathbf H_1$ as $\mathbf{H}^{{-1}}=\mathbf{V}_1{\mathbf{\Sigma}^{-1}}_m \mathbf{U}_\mathbf{H}^{\dagger}$.
\item Take $(-\mathbf{S}_m)$ as the non-positive eigenmodes of $\mathbf{H}_1\mathbf{D}_1^{-1}\mathbf{H}_1^{\dagger}-\mathbf{I}_m$.
\item $\mathbf{Z}=\mathbf{H}^{-1}\mathbf{S}_m(\mathbf{H}^{-1})^{\dagger}$.
\item $\mathbf{B} = \mathbf{V}_1^{\dagger}\left(\mathbf{Z}-\mathbf{H}^{-1}(\mathbf{H}^{-1})^{\dagger}\right)\mathbf{D}_1\mathbf{V}_2(\mathbf{V}_2^{\dagger}\mathbf{D}_1\mathbf{V}_2)^{-1}$.
\item
$\mathbf{A}=\left(\mathbf{I}_{n-m}-\mathbf{B}^{\dagger}\mathbf{V}_1^{\dagger}\mathbf{D}_1\mathbf{V}_2\right)(\mathbf{V}_2^{\dagger}\mathbf{D}_1\mathbf{V}_2)^{-1}$.
\item
$\mathbf{X}=\mathbf{V}_2\mathbf{A}\mathbf{V}_2^{\dagger}+\mathbf{V}_1\mathbf{B}\mathbf{V}_2^{\dagger}+\mathbf{V}_2\mathbf{B}\mathbf{V}_1^{\dagger}$.
\item
$\mathbf{Q}_{1}^{\ast}=\mathbf{D}_1^{-1}-\mathbf{H}^{-1}(\mathbf{H}^{-1})^{\dagger}+\mathbf{Z}-\mathbf{X}$.
\end{itemize}

\item \emph{Update $\mathbf D_1$}: $\mathbf{D}_{1}^{\mathrm{-1}}\leftarrow \mathbf{D}_1^{{-1}}+\mathbf{P}_{1}-\text{diag} (\mathbf{Q}_1^{\ast})$.
\end{enumerate}
After choosing an initial $\mathbf{D}_1\succ \mathbf 0$,
the above procedure is repeated until the duality gap $|\text{tr}(\mathbf{D}_{1}(\mathbf{Q}_{1}^{\ast}-\mathbf{P}_{1}))|$ converges to within a pre-specified tolerance. 
The algorithm is shown to always converge to the optimal value. For more details on the derivation and convergence analysis, refer to \cite{vu2011capacity}.


%To adaptively obtain the optimal $\mathbf{Q}_{1}^{\ast}$, we choose an initial $\mathbf{D}_1^{0}\succ \mathbf 0$ and adjust it iteratively. At $i$th iterative procedure, we have obtained $\mathbf{D}_1^{i}$  and perform the following updates:
%\begin{IEEEeqnarray}{rCl}
%\label{singleusermodedropping n>=m} 
%-\mathbf{S}_n^{i}&=&\text{non-positive eigenmodes of } \mathbf{K}(\mathbf{D}_1^{i})^{-1}\mathbf{K}^{\dagger}-\mathbf{I}_n \nonumber\\
%\mathbf{Z}^{i}&=&\mathbf{K}^{-1}\mathbf{S}_n^{i}(\mathbf{K}^{-1})^{\dagger}\nonumber \\
%\mathbf{Q}_{1}^{i}&=&(\mathbf{D}_1^{i})^{-1}-\mathbf{K}^{-1}(\mathbf{K}^{-1})^{\dagger}+\mathbf{Z}^{i} \nonumber \\
%\mathbf{D}_{1}^{i+1}&=&\mathbf{D}_1^{i}+\mathbf{P}-\text{diag} (\mathbf{Q}_1^{i})
%\end{IEEEeqnarray}
%The updates stops when the duality gap is close to $0$ within an acceptable tolerance.


%For $n>m$, we define the channel ``inverse'' $\mathbf{H}^{-1}=\mathbf{V}_1{\Sigma}_m \mathbf{U}_\mathbf{H}^{\dagger}$, where $\mathbf{V}_1$ is the first $m$ columns of $\mathbf{V}_\mathbf{H}$ ($\mathbf{V}_\mathbf{H}=[\mathbf{V}_1\text{ } \mathbf{V}_2]$) and ${\mathbf{\Sigma}}_m$ is $m\times m$ diagonal matrix containing the non-zero singular values of $\mathbf{H}_1$. It is stated by Theorem 2 of \cite{vu2011capacity}, the optimal $\mathbf{Q}_{1}^{\ast}$ satisfying the optimality conditions (\ref{singleKKT1}) is given by $\mathbf{Q}_{1}^{\ast}=\mathbf{D}_1^{-1}-\mathbf{H}^{-1}(\mathbf{H}^{-1})^{\dagger}+\mathbf{Z}-\mathbf{X}$, where $\mathbf{Z}=\mathbf{H}^{-1}\mathbf{S}_m(\mathbf{H}^{-1})^{\dagger}$ and $(-\mathbf{S}_m)$ is the non-positive eigenmodes of $\mathbf{H}\mathbf{D}_1^{-1}\mathbf{H}^{\dagger}-\mathbf{I}_m$. Here $\mathbf{X}=\mathbf{V}_2\mathbf{A}\mathbf{V}_2^{\dagger}+\mathbf{V}_1\mathbf{B}\mathbf{V}_2^{\dagger}+\mathbf{V}_2\mathbf{B}\mathbf{V}_1^{\dagger}$, where $\mathbf{A}$ and $\mathbf{B}$ are given by, respectively
%\begin{IEEEeqnarray}{rCl}
%\label{singleusermodedropping AB} 
%\mathbf{B}&=&\mathbf{V}_1^{\dagger}\left(\mathbf{Z}-\mathbf{H}^{-1}(\mathbf{H}^{-1})^{\dagger}\right)\mathbf{D}_1\mathbf{V}_2(\mathbf{V}_2^{\dagger}\mathbf{D}_1\mathbf{V}_2)^{-1} \nonumber \\
%\mathbf{A}&=&\left(\mathbf{I}_{n-m}-\mathbf{B}^{\dagger}\mathbf{V}_1^{\dagger}\mathbf{D}\mathbf{V}_2\right)(\mathbf{V}_2^{\dagger}\mathbf{D}_1\mathbf{V}_2)^{-1}
%\end{IEEEeqnarray}

%Therefore, the optimal $\mathbf{Q}_{1}^{\ast}$ can be found in the similar manner to the case when $n \leq m$.
%Having obtained $\mathbf{D}_1^{i}$ at $i$th iterative procedure, the following update are performed:
%\begin{IEEEeqnarray}{rCl}
%\label{singleusermodedropping n<m} 
%-\mathbf{S}_m^{i}&=&\text{non-positive eigenmodes of } \mathbf{H}(\mathbf{D}_1^{i})^{-1}\mathbf{H}^{\dagger}-\mathbf{I}_m \nonumber\\
%\mathbf{Z}^{i}&=&\mathbf{H}^{-1}\mathbf{S}_m^{i}(\mathbf{H}^{-1})^{\dagger}\nonumber \\
%\mathbf{X}^{i}&=&\mathbf{V}_2\mathbf{A}^{i}\mathbf{V}_2^{\dagger}+\mathbf{V}_1\mathbf{B}_i\mathbf{V}_2^{\dagger}+\mathbf{V}_2\mathbf{B}_i\mathbf{V}_1^{\dagger}\nonumber \\
%\mathbf{Q}_{1}^{i}&=&(\mathbf{D}_1^{i})^{-1}-\mathbf{H}^{-1}(\mathbf{H}^{-1})^{\dagger}+\mathbf{Z}^{i}-\mathbf{X}^{i} \nonumber \\
%\mathbf{D}_{1}^{i+1}&=&\mathbf{D}_1^{i}+\mathbf{P}-\text{diag} (\mathbf{Q}_1^{i})
%\end{IEEEeqnarray}
%Finally, the duality gap goes to zero and the algorithm converges to the optimal solution. It was shown analytically that the algorithm always converges to the optimal value. The convergence rate is observed numerically to be exponentially fast.
%Details can be found in \cite{vu2011capacity}. 




The capacity of single-user MISO channels with per-antenna constraint is a special case of $n> m$ in which $m=1$ and the channel matrix $\mathbf{H}_1$ reduces to a vector $\mathbf{h}_1\in \mathbf{C}^{1\times n}$. In this case, closed-form optimal solution exists and no iterative procedure is necessary \cite{vu2011miso}. The entries of optimal covariance matrix are given by
\begin{equation}
q_{ij}=\frac{h_{1i}^*h_{1j}}{|h_{1i}h_{1j}|}\sqrt{P_{1i}P_{1j}}, \quad  i,j=1,\cdots,n.
\end{equation}
where the $h_{1i}$ is the $i$th entry of channel vector $\mathbf{h}_1$.

%According to the results in \cite{vu2011miso}, the MISO capacity under per-antenna power constraint can be expressed as
%\begin{IEEEeqnarray}{rCl}
%\label{MISOcapacity} 
%C_{\text{MISO}} = \log \left[1+\left(\sum_{j=1}^{n}|h_{1j}|\sqrt{P_{1j}}\right)^2\right]
%\end{IEEEeqnarray}
%where $h_{1j}$ is $j$th entry of the channel matrix $\mathbf{h}_1$.

 
\subsection{Iterative mode-dropping}
The following theorem on the optimality conditions motivates and lays the foundation for the iterative mode-dropping algorithm:

\begin{theorem}[Optimality conditions]
\label{theorem:opt}
The set of transmit covariance matrices, $\{\mathbf{Q}^{\ast}_i\}$, is the optimal solution of the MIMO-MAC sum-rate maximization problem in (\ref{perantennapowerMAC}) \emph{if and only if} 
for each  $i \in \{1,\cdots, K\}$, $\mathbf{Q}^{\ast}_i$ is the optimal solution of the single-user rate maximization problem:
\begin{IEEEeqnarray}{rCl}
\label{singleusermodedropping} 
\max \quad&&\log \det (\mathbf{I}_m+\mathbf{\hat{H}}_i\mathbf{Q}_i\mathbf{\hat{H}}_i^{\dagger})  \\
\mathrm{s.t.} \quad&&\mathrm{diag}(\mathbf{Q}_i) \preccurlyeq \mathbf{P}_i\nonumber \\
&&\mathbf{Q}_i \succcurlyeq \mathbf 0  \;, \nonumber
\end{IEEEeqnarray}
where $\mathbf{\hat{H}}_i$ is the effective channel matrix defined as
\begin{IEEEeqnarray}{rCl}
\label{effectivechannel} 
 \mathbf{\hat{H}}_i=\Big(\mathbf{I}_m+\sum_{k=1,k \neq i}^{K}\mathbf{H}_{k}\mathbf{Q}_{k}^{\ast}\mathbf{H}_{k}^{\dagger}\Big)^{-1/2}\mathbf{H}_i\;.
\end{IEEEeqnarray}
\end{theorem}
\begin{IEEEproof}
The \emph{only if} part is easy and follows similar argument to the proof of Theorem 1 in \cite{yu2004iterative}. 
Herein, we prove the \emph{if} part. 
From the KKT conditions of the multiuser problem in (\ref{perantennapowerMAC}),
we can obtain a set of necessary and sufficient optimality conditions as 
%The \emph{if} part follows from the KKT conditions of the sum-rate problem in
%(\ref{perantennapowerMAC}) which are
%\begin{IEEEeqnarray}{rCl}
%\label{multiLagrangian} 
%\mathcal{L}(\mathbf{Q}_i,\mathbf{D}_i,\mathbf{M}_i&&)=\log \det(\mathbf{I}_m+\sum_{i=1}^{K}\mathbf{H}_i\mathbf{Q}_i\mathbf{H}_i^{\dagger}) \nonumber \\
%&& - \sum_{i=1}^{K}\text{tr}[{(\mathbf{D}_i(\mathbf{Q}_i-\mathbf{P}_i)}]+\sum_{i=1}^{K}\text{tr}(\mathbf{M}_i\mathbf{Q}_i)\;, \quad
%\end{IEEEeqnarray}
%Follow the steps in \cite{vu2011capacity}, the multiuser KKT conditions are obtained
\begin{IEEEeqnarray}{rCl}
\label{multiKKT} 
\label{multiKKT1}
\mathbf{H}_i^{\dagger} \Big(\mathbf{I}_m+\sum_{i=1}^{K}\mathbf{H}_i\mathbf{Q}_i ^{\ast}\mathbf{H}_i^{\dagger} \Big)^{-1}\mathbf{H}_i&=&\mathbf{D}_i-\mathbf{M}_i  \\
\label{multiKKT2}
\mathbf{M}_i\mathbf{Q}_i^{\ast}&=&\mathbf{0} \nonumber \\
\label{multiKKT3} 
\text{diag}(\mathbf{Q}_i^{\ast})&=&\mathbf{P}_i \nonumber \\
\label{multiKKT4}
\mathbf{M}_i,\mathbf{Q}_i^{\ast} &\succcurlyeq& \mathbf 0 \nonumber \\
\text{diagonal } \mathbf{D}_i&\succ& \mathbf 0 \nonumber \;,
\end{IEEEeqnarray}
for all $i=1,2\cdots,K$. 
The matrices $\{ \mathbf M_i \}$ and $\{ \mathbf D_i \}$ are dual variables associated with the per-antenna power constraints of the $K$ users and the positive semidefinite constraints of the covariance matrices.
Using similar arguments to the single-user case, a set of covariance matrices satisfying these conditions is the optimal solution of the MIMO-MAC problem. 

%The matrix $\mathbf{D}_i$ is the dual variable associated with the per-antenna power constraint of user $i$. 
%It is strictly positive since at optimum, $\text{diag}(\mathbf{Q}_i)=\mathbf{P}_i$ for all $i=1,2\cdots,K$, otherwise we can always increase the power of antennas to obtain a higher sum rate. 
%The matrix $\mathbf{M}_i$ is the dual variable associated with the positive semidefinite constraint. Because the problem is convex, the KKT conditions are also sufficient and thus the set $\{\mathbf{Q}_i\}$ satisfying all these conditions is the optimal solution of the sum-rate maximization problem. 

Next, we decouple the conditions in \eqref{multiKKT} into an equivalent ensemble of 
$K$ single-user optimality conditions.
This can be done by rewriting the first equation in (\ref{multiKKT}) as
\begin{IEEEeqnarray}{rCl}
\label{multiKKTstep2}
\mathbf{\hat{H}}_i^{\dagger} (\mathbf{\mathbf{I}_m+\hat{H}}_{i}\mathbf{Q}_i^{\ast}\mathbf{\hat{H}}_{i}^{\dagger})^{-1}\mathbf{\hat{H}}_i=\mathbf{D}_i-\mathbf{M}_i\;,
\end{IEEEeqnarray}
where $\mathbf{\hat{H}}_i$ is the effective channel matrix defined in (\ref{effectivechannel}). 
It follows that  $\text{rank}(\mathbf{\hat{H}}_i)=\text{rank}(\mathbf{H}_i)$.  
%  $\mathbf{\hat{H}}_i \in \mathbb{C}^{m\times n}$ is of full column (or row) rank. 
%This condition combined with the complementary slackness and primary and dual constraints for $i$th user reduce to the standard single-user KKT condition in \cite{vu2011capacity} with the physical channel matrix $\mathbf{H}_i$ replaced by the effective channel matrix $\mathbf{\hat{H}}_i$. The problem is convex, thus the KKT condition is sufficient and necessary. The covariance matrix $\{\mathbf{Q}_i\}$ ($\mathbf{Q}_i$) satisfies multiuser KKT conditions (single-user KKT conditions) are the solutions of multiuser (single-user) problem.
By replacing the first equation in (\ref{multiKKT}) by (\ref{multiKKTstep2}), the multiuser optimality conditions are successfully decoupled. 

In turn, the new conditions with (\ref{multiKKTstep2}) for each $i$ are exactly the optimality conditions for the single-user rate maximization problems in \eqref{singleusermodedropping}.
That is,
 if for each $i \in \{1, \cdots, K\}$, $\mathbf{Q}_i^\ast$ is the optimal solution of \eqref{singleusermodedropping},
then the set $\{ \mathbf Q_i^\ast \}$ will automatically satisfy the multiuser optimality conditions in (\ref{multiKKT}), 
and is therefore the optimal solution of the sum-rate problem in (\ref{perantennapowerMAC}).
\end{IEEEproof}

Theorem~\ref{theorem:opt}  uncovers a simple but interesting fact: 
the optimal transmit covariance matrices, $\{ \mathbf Q_{i}^{\ast} \}$,
are in a state of equilibrium.
The process of finding them can be viewed as
that of moving towards this equilibrium state.
The iterative mode-dropping algorithm successively optimizes one of these matrices at a time,
while maintaining the others, 
and in the end reaches the equilibrium.
The procedure is given in Algorithm 1.

\begin{algorithm}
Initialize $\mathbf{Q}_i=\mathbf{0}$, $i=1,\cdots,K$ \\
$\mathbf{repeat}$\\
\quad for $i=1,\cdots, K$\\
\quad \qquad $\mathbf{W}_z^{(i)}=\mathbf{I}_m+\sum_{k=1,k \neq i}^{K}\mathbf{H}_{k}\mathbf{Q}_{k}\mathbf{H}_{k}^{\dagger}$\\
\quad \qquad  $\mathbf{\hat{H}}_i=\left(\mathbf{W}_z^{(i)}\right)^{-1/2}\mathbf{H}_i$\\
\quad \qquad  $\mathbf{Q}_i = \underset{{\text{diag}(\mathbf{Q})\preccurlyeq \mathbf{P}_i, \mathbf{Q} \succcurlyeq 0}}{\arg\max}  \log \det (\mathbf{\hat{H}}_{i}\mathbf{Q}\mathbf{\hat{H}}_{i}^{\dagger}+\mathbf{I}_m)$\\
 \quad \qquad (using single-user mode-dropping in Section III.A) \\
\quad end\\
$\mathbf{until\text{ }the\text{ }sum\text{ }rate\text{ }converges}$
\caption{Iterative mode-dropping for MIMO-MAC sum-rate maximization with per-antenna power constraint}
\end{algorithm}

The following theorem establishes the sure convergence of the proposed algorithm:
\begin{theorem}[Convergence]
In iterative mode-dropping for MIMO-MAC, the sum rate always converges to the sum capacity and all the covariance matrices $\{\mathbf{Q}_i\}$ converge to the optimal matrices.
\end{theorem}
\begin{IEEEproof}
%At the $i$th step, the single-user mode-dropping algorithm finds the optimal $\mathbf Q_{i}$ to maximize the sum rate while keeping the covariance matrices of all other users unaltered. 
%Henceforth, the sum rate is nondecreasing at each step.
%Since the sum rate is always bounded above for a finite power budget,
%it always converges to a limit $C$.
%
%Next, we prove by contradiction that $C$ is exactly the sum capacity.
%% achieved by the optimal  transmit covariance matrices $\{\mathbf{Q}_i^{\mathrm o}\}$.
%If $C$ is not,  we let $C^{\prime} > C$ be the true sum capacity.
%Since the sum rate is a continuous, strictly concave function of $\{\mathbf Q_{i} \}$, 
%there must exists at least a set of $\{ \bar{\mathbf Q}_{i} \}$
%such that the sum rate is $C$.
%
%The transmit covariance matrices $\{\mathbf{Q}_i\}$ also converge to the optimal matrices.
%
%================
At the $i$th step of each iteration,  single-user mode-dropping finds the optimal $\mathbf Q_{i}$ to maximize the sum rate while keeping the other covariance matrices unchanged. 
Since the objective function of this subproblem is continuous and strictly concave, 
the optimal solution is unique and
the optimized covariance matrix either remains unaltered or changes to increase the sum rate. 
Henceforth, the sum rate is nondecreasing at each step.
Furthermore, it is always bounded above for a finite power budget. 
Hence the sum rate must converge to a limit.
%Due to the continuity, this limit will at least be achieved by a set of $\mathbf Q_i^{\mathrm o}$.
In addition, 
the sum rate is also a continuous function of $\mathbf Q_i$.
Therefore, as the sum rate approaches the sum capacity,
the changes in $\mathbf Q_i$ diminish. 
In the end,
each covariance matrix converges to the solution of the single-user problem in \eqref{singleusermodedropping}.
 According to Theorem 1,  the proof is complete.
%, this limit is the sum capacity and all the covariance matrices $\{\mathbf{Q}_i\}$ converge to the optimal matrices.
\end{IEEEproof}

%\begin{corollary}
%After one iteration of Algorithm 1, the sum-rate objective is at most $(K-1)m/2$ nats away from the sum capacity, provided that the duality gap in single-user mode-dropping approaches zero.
%\end{corollary}
%\begin{IEEEproof}
%The proof is similar to the proof of Theorem 3 in \cite{yu2004iterative} and we only highlight the difference. The term $\lambda_iP_i$ is replaced by $\mathbf{D}_i\mathbf{P}_i$ here and $\mathbf{S}_z$ is replaced by $\mathbf{I}_m$. To illustrate that the multiuser duality gap is bounded by $(K-1)m/2$, Ref.~\cite{yu2004iterative} proved that $\lambda_i\leq\lambda_i'$.
%Here, instead, we need to show that $\text{tr}(\mathbf{D}_i\mathbf{P_i})\preccurlyeq \text{tr}(\mathbf{D}'_i\mathbf{P_i})$ for all $i=1,2,\cdots,K$, where diagonal matrix $\mathbf{D}_i$ is the solution of the following minimization problem,
%\begin{IEEEeqnarray}{rCl}
%\label{D_iOptimization} 
%\min \quad&&\text{tr}(\mathbf{D}_i\mathbf{P}_i)\nonumber \\
%\text{s.t.} \quad &&\mathbf{D}_i \succcurlyeq \mathbf{H}_{i}^{\dagger}\mathbf{Z}_K^{-1}\mathbf{H}_{i}\quad \;,
%\end{IEEEeqnarray}
%and diagonal matrix $\mathbf{D}'_i$ is the solution of the following minimization problem
%\begin{IEEEeqnarray}{rCl}
%\label{D_i'Optimization} 
%\min \quad&&\text{tr}(\mathbf{D}'_i\mathbf{P}_i)\nonumber \\
%\text{s.t.} \quad &&\mathbf{D}'_i \succcurlyeq \mathbf{H}_{i}^{\dagger}\mathbf{Z}_i^{-1}\mathbf{H}_{i}\;.\quad  
%\end{IEEEeqnarray}
%where $\mathbf{Z}_i=\sum_{k=1}^{i}\mathbf{H}_k\mathbf{Q}_k\mathbf{H}_{k}^{\dagger}+\mathbf{I}_m$.
%Since
%\begin{IEEEeqnarray}{rCl}
%\label{Hinequality} 
%\mathbf{H}_{i}^{\dagger}\mathbf{Z}_K^{-1}\mathbf{H}_{i}\preccurlyeq \mathbf{H}_{i}^{\dagger}\mathbf{Z}_i^{-1}\mathbf{H}_{i} \quad  i=1,2,\cdots,K\;, 
%\end{IEEEeqnarray}
%the feasible region of optimization problem in (\ref{D_iOptimization}) includes that in (\ref{D_i'Optimization}) as a subset. Thus at optimum, we have $\text{tr}(\mathbf{D}_i\mathbf{P_i})\preccurlyeq \text{tr}(\mathbf{D}'_i\mathbf{P_i})$. This holds for all $i=1,2,\cdots,K$.
%\end{IEEEproof}

%\emph{Remark}~1: In fact,  iterative mode-dropping is a block coordinate descent (or ascent) method.
%Because the sum-rate objective is a continuous, strictly concave function of $\{ \mathbf Q_{i} \}$,
%iterative mode-dropping must converge to the optimal point \cite{Luo1992}.
\emph{Remark}~1: 
Iterative water-filling  and iterative mode-dropping update $\{ \mathbf Q_{i} \}$  differently.
At each step of iterative water-filling, 
the eigenvectors of $\mathbf Q_{i}$ are solely determined by the left singular vectors of corresponding effective channel matrix and do not depend on the SNR of the $i$th user.
The eigenvalues of $\mathbf Q_{i}$ are then found by water-filling the total power across the spatial subchannels. 
In contrast, for iterative mode-dropping,
both the eigenvectors and eigenvalues of the optimal $\mathbf Q_{i}$ depend not only on the effective channel matrix but also on the SNR
and the power constraint.
This is because with per-antenna power constraint,
the optimal $\mathbf Q_i$ is not diagonalizable by the left singular vectors of the effective channel matrix.
Thus in each step, iterative mode-dropping usually updates both the eigenvectors and eigenvalues of $\mathbf Q_i$ simultaneously.


% To Mai Vu:
%I did not include the sentence "In iterative water-filling, at each steps the eigenvectors of Qi can be found analytically independent of the SNR and the algorithm only updates the eigenvalues of Qi (or the lambda_i). " It is true that the waterfilling processes does not update the eigenvectors of Qi. But this might make people think that the eigenvectors do not change from iteration to iteration, which is generally not true because the effective channel matrices in (7) are changing because the Q's are changing from iteration to iteration.


%at each steps the eigenvectors of $\mathbf Q_{i}$ can be found analytically independent of the SNR and the algorithm only updates the eigenvalues of Qi (or the $\lambda_i$). 
%But in iterative mode-dropping, the algorithm usually updates both the eigenvectors and eigenvalues of Qi simultaneously. The reason is with per-antenna power constraint, the optimal covariance solution is not diagonalizable by the channel singular vectors and often has both the eigenvectors and eigenvalues dependent on the SNR and the power 


\emph{Remark}~2: The convergence in Theorem 2 holds for all random channel realizations. Although Theorem 2 holds for arbitrary initial conditions, 
setting initial covariance matrices to zero provides a fast convergence. More specifically,  the sum rate is at most $(K-1)m/2$ nats away from the sum capacity after only one iteration for every $\mathbf Q_{i}$.
This is the same as the rate of convergence for iterative water-filling.
%provided that the duality gap in single-user mode-dropping approaches zero. 
Since the proof follows the same procedure as the proof for Theorem 3 in \cite{yu2004iterative}, we only highlight here the difference. 
The terms $\lambda_iP_i$ and $\mathbf{S}_z$ in \cite{yu2004iterative} are replaced by $\text{tr}(\mathbf{D}_i\mathbf{P_i})$ and $\mathbf{I}_m$, respectively. To illustrate that the multiuser duality gap is bounded by $(K-1)m/2$, the authors of \cite{yu2004iterative} proved that the dual variables $\lambda_i\leq\lambda_i'$.
Here, instead, we need to show that $\text{tr}(\mathbf{D}_i\mathbf{P_i})\preccurlyeq \text{tr}(\mathbf{D}'_i\mathbf{P_i})$ for all $i=1,2,\cdots,K$, where diagonal matrix $\mathbf{D}_i$ is the solution of the following minimization problem:
\begin{IEEEeqnarray}{rCl}
\label{D_iOptimization} 
\min \quad&&\text{tr}(\mathbf{D}_i\mathbf{P}_i)\nonumber \\
\text{s.t.} \quad &&\mathbf{D}_i \succcurlyeq \mathbf{H}_{i}^{\dagger}\mathbf{W}_K^{-1}\mathbf{H}_{i}\, \;,
\end{IEEEeqnarray}
and diagonal matrix $\mathbf{D}'_i$ is the solution of the following minimization problem:
\begin{IEEEeqnarray}{rCl}
\label{D_i'Optimization} 
\min \quad&&\text{tr}(\mathbf{D}'_i\mathbf{P}_i)\nonumber \\
\text{s.t.} \quad &&\mathbf{D}'_i \succcurlyeq \mathbf{H}_{i}^{\dagger}\mathbf{W}_i^{-1}\mathbf{H}_{i}\;,\quad  
\end{IEEEeqnarray}
where $\mathbf{W}_i=\sum_{k=1}^{i}\mathbf{H}_k\mathbf{Q}_k\mathbf{H}_{k}^{\dagger}+\mathbf{I}_m$.
Indeed, because
\begin{IEEEeqnarray}{rCl}
\label{Hinequality} 
\mathbf{H}_{i}^{\dagger}\mathbf{W}_K^{-1}\mathbf{H}_{i}\preccurlyeq \mathbf{H}_{i}^{\dagger}\mathbf{W}_i^{-1}\mathbf{H}_{i} , \quad \forall  i=1,2,\cdots,K\;, 
\end{IEEEeqnarray}
the feasible region of the optimization problem in (\ref{D_iOptimization}) includes that of (\ref{D_i'Optimization}) as a subset. Therefore, at optimum, we have $\text{tr}(\mathbf{D}_i\mathbf{P_i})\preccurlyeq \text{tr}(\mathbf{D}'_i\mathbf{P_i})$, which holds for all $i=1,2,\cdots,K$.

\emph{Remark}~3: 
%The proposed algorithm has complexity that increases almost linearly with the number of users $K$. In each iteration, each user's effective channel matrix is calculated and its covariance matrix is optimized using single-user mode-dropping with the effective channel successively. For multiple numerical examples, the single-user mode-dropping converges exponentially fast independent of the number of users. This desirable property does not exist for general optimization methods such as standard interior point methods whose complexity is cubic with respect to the input dimensionality. 
The computational complexity of iterative mode-dropping 
is approximately the product of the expected complexity of single-user mode-dropping, the number of iterations and
the number of users $K$.
We found from numerous numerical experiments that the former two almost do not change and
therefore, the total complexity scales linearly with $K$ as shown later in simulations (Figure~\ref{complexity}).
In contrast, the complexity of interior-point methods is a cubic function of $K$ \cite{Boyd2004}.
This improvement becomes more significant when the number of users $K$ increases. 



\emph{Remark}~4: Although the proposed algorithm successfully calculates the sum capacity of MIMO-MAC under per-antenna power constraint, it cannot be used directly 
to generate the whole capacity region except the inner and outer bounds as shown in Section IV. 
To obtain the whole region, one needs to solve the following weighted sum-rate maximization problem: 
\begin{IEEEeqnarray}{rCl}
\label{perantennapowerMAC1} 
\max_{\{\mathbf{Q}_i\}} \quad&&\sum_{j=1}^K \omega_{\pi_j} \log \det \Big(\frac{\mathbf{I}_m+\sum_{i=1}^{j}\mathbf{H}_{\pi_{i}}\mathbf{Q}_{\pi_{i}}\mathbf{H}_{\pi_{i}}^{\dagger}}{\mathbf{I}_m+\sum_{i=1}^{j-1}\mathbf{H}_{\pi_{i}}\mathbf{Q}_{\pi_{i}}\mathbf{H}_{\pi_{i}}^{\dagger}}\Big)  \\
\text{s.t.} \quad&&\text{diag}(\mathbf{Q}_i) \preccurlyeq \mathbf{P}_i, \quad i=1,\cdots,K\nonumber \\
&&\mathbf{Q}_i \succcurlyeq \mathbf 0,\quad \quad \quad\quad i=1,\cdots,K \nonumber \;,
\end{IEEEeqnarray}
where $\pi_{i}$ denotes decoding order (the user $\pi_{K}$ is decoded first and user $\pi_{1}$ decoded last) and the weights satisfy $\omega_{\pi_1}\geq \omega_{\pi_2}\geq \cdots \geq \omega_{\pi_K}$.
Efficient solution for this weighted-sum-rate problem up to now is still unclear, even under the sum power constraint. 





==> mathdef2010.tex <==
% Mathematical environments:
\def\BD{\begin{displaymath}}
\def\BEA{\begin{eqnarray}}
\def\BEAs{\begin{eqnarray*}}
\def\ED{\end{displaymath}}
\def\EEA{\end{eqnarray}}
\def\EEAs{\end{eqnarray*}}

% Boldface Characters:
\def\bA{{\bf A}}
\def\ba{{\bf a}}
\def\bB{{\bf B}}
\def\bb{{\bf b}}
\def\bC{{\bf C}}
\def\bc{{\bf c}}
\def\bD{{\bf D}}
\def\bd{{\bf d}}
\def\bE{{\bf E}}
\def\be{{\bf e}}
\def\bF{{\bf F}}
%\def\bf{{\bf f}}
\def\bG{{\bf G}}
\def\bg{{\bf g}}
\def\bH{{\bf H}}
\def\bh{{\bf h}}
\def\bI{{\bf I}}
\def\bJ{{\bf J}}
\def\bK{{\bf K}}
\def\bk{{\bf k}}
\def\bM{{\bf M}}
\def\bL{{\bf L}}
\def\bN{{\bf N}}
\def\bn{{\bf n}}
\def\bP{{\bf P}}
\def\bp{{\bf p}}
\def\bq{{\bf q}}
\def\bQ{{\bf Q}}
\def\bR{{\bf R}}
\def\br{{\bf r}}
\def\bS{{\bf S}}
\def\bs{{\bf s}}
\def\bT{{\bf T}}
\def\bU{{\bf U}}
\def\bu{{\bf u}}
\def\bV{{\bf V}}
\def\bv{{\bf v}}
\def\bW{{\bf W}}
\def\bw{{\bf w}}
\def\bX{{\bf X}}
\def\bx{{\bf x}}
\def\bY{{\bf Y}}
\def\by{{\bf y}}
\def\bZ{{\bf Z}}
\def\bz{{\bf z}}
\def\bzero{\bm 0}
\def\bone{\bm 1}

% Boldface greek:
% Note package bm.sty must be used: \usepackage{bm}
%\def\balpha{\bm{\alpha}}
\def\balpha{\mbox{\boldmath $\alpha$}}
\def\bDelta{\mbox{\boldmath $\Delta$}}
\def\beps{\mbox{\boldmath $\epsilon$}}
\def\b_eta{\mbox{\boldmath $\eta$}}
\def\bGamma{\mbox{\boldmath $\Gamma$}}
\def\bkappa{\mbox{\boldmath $\kappa$}}
\def\bLambda{\mbox{\boldmath $\Lambda$}}
\def\bnu{\mbox{\boldmat $\nu$}}
\def\bomega{\mbox{\boldmath $\omega$}}
\def\bOmega{\bm{\Omega}}
\def\bPhi{\mbox{\boldmath $\Phi$}}
\def\bphi{\mbox{\boldmath $\phi$}}
\def\bPsi{\mbox{\boldmath $\Psi$}}
\def\bpsi{\mbox{\boldmath $\psi$}}
\def\bSigma{\mbox{\boldmath $\Sigma$}}
\def\bsigma{\mbox{\boldmath $\sigma$}}
\def\bTheta{\mbox{\boldmath $\Theta$}}
\def\btheta{\mbox{\boldmath $\theta$}}
\def\bmu{\bm{\mu}}
\def\bxi{\bm{\xi}}


% Caligraphy Characters:
\def\mcA{\mathcal{A}}
\def\mcB{\mathcal{B}}
\def\mcC{\mathcal{C}}
\def\mcD{\mathcal{D}}
\def\mcE{\mathcal{E}}
\def\mcF{\mathcal{F}}
\def\mcG{\mathcal{G}}
\def\mcX{\mathcal{X}}
\def\mcK{\mathcal{K}}
\def\mcH{\mathcal{H}}
\def\mcI{\mathcal{I}}
\def\mcL{\mathcal{L}}
\def\mcM{\mathcal{M}}
\def\mcN{\mathcal{N}}
\def\mcP{\mathcal{P}}
\def\mcQ{\mathcal{Q}}
\def\mcR{\mathcal{R}}
\def\mcS{\mathcal{S}}
\def\mcT{\mathcal{T}}
\def\mcU{\mathcal{U}}
\def\mcW{\mathcal{W}}
\def\mcZ{\mathcal{Z}}
\def\mcE{\mathcal{E}}

% Boldface caligraphy characters:
\def\bcA{\mbox{\boldmath ${\cal A}$}}

% Mathematical set characters:
\newcommand{\msC}{\mathbb{C}}
\def\msI{{\mathbb{I}}}
\def\msN{{\mathbb{N}}}
\def\msR{{\mathbb{R}}}
\def\msZ{{\mathbb{Z}}}

% Frequently used operators:
\def\diag{{\rm diag}}
\def\dist{{\rm dist}}
\def\Imag{\mbox{Im}}
\def\Real{\mbox{Re}}
\def\trace{{\rm tr}}

% Useful abbreviations:
\def\eps{\epsilon}
\def\om{\omega}

% Others possible definitions:
\def\txi{{\tilde \xi}}
\def\ul{\underline}
\def\cspan{\mathop{\rm span} \nolimits}
%\def\Tr{{\rm tr}}
\def\sinc{{\rm sinc}}
\def\define{\buildrel \triangle \over =}
\def\spn{{\rm Span}}
\def \Cset    {\hbox{\hskip 2pt { I} \hskip -1.5pt \llap{C}}}
\def\bull{\vrule depth -.1ex
                 width .8ex
                 height .9ex}
\def\tvert{\vert \hskip -1pt \Vert}
\def\L2{L^{2}[-{\pi \over 2} , {\pi \over 2}]}
\def\integ{\int_{-{\pi \over 2}}^{{\pi \over 2}}}
\def\bt{\btheta}
\def\bnu{\bnu}
\def\ct{\hat{\btheta}}
\def\tk{\btheta^{k}}
\def\tki{\btheta^{k}_{i-1}}
\def\htk{\hat{\btheta}^{k}}
\def\htki{\hat{\btheta}^{k}_{i-1}}
\def\hR{\hat{\bf R}}
\def\brR{\bar{\bf R}}
\def\bRk{{\bf R}^{k}}
\def\hRk{\hat{{\bf R}}^{k}}
\def\hRki{\hat{{\bf R}}^{k}_{i-1}}
\def\Rki{{\bf R}^{k}_{i-1}}
\def\hs{\hat{\sigma}^{2}}
\def\hsk{\hat{\sigma}^{2}_{k}}
\def\hp{\hat{\psi}}
\def\RTCT{{\bf R}_{\rm TCT}}
\def\ECSM{{\cal E}_{\rm CSM}}
\def\ETCT{{\cal E}_{\rm TCT}}
\def\PCSM{\bPhi_{\rm CSM}}
\def\PTCT{\bPhi_{\rm TCT}}
\def\AIC{{\rm AIC}}
\def\MDL{{\rm MDL}}
\def\PSC{{\rm P\hspace{-.1em}S\hspace{-.1em}C}}
%\def\proof{{\bf Proof:}}
%\def\SNReq{{\rm SNR}_{eq}}
%\def\SNRth{{\rm SNR}_{th}}

